A Problem-Oriented Perspective and Anchor Verification for Code Optimization

Large Language Models (LLMs) have shown remarkable capabilities in solving various programming tasks, such as code generation. However, their potential for code optimization, particularly in performance enhancement, remains largely unexplored. This paper investigates the capabilities of LLMs in optimizing code for minimal execution time, addressing a critical gap in current research. The recently proposed code optimization methods construct program optimization pairs based on iterative submissions from the same programmer for the same problem. However, this approach confines LLMs to local performance improvements, neglecting global algorithmic innovation. To overcome this limitation, we adopt a completely different perspective by reconstructing the optimization pairs into a problem-oriented approach. This allows for the integration of various ideas from multiple programmers tackling the same problem. Furthermore, we observe that code optimization presents greater challenges compared to code generation, often accompanied by "optimization tax". Recognizing the inherent trade-offs in correctness and efficiency, we introduce a novel anchor verification framework to mitigate this "optimization tax". Ultimately, the problem oriented perspective combined with the anchor verification framework significantly enhances both the correct optimization ratio and speedup to new levels.

==> tables/anchor.tex <==
\begin{table*}[!htb]
    \centering
    \small
     \caption{Results of Anchor Verification and compared methods with \qwencoder, GPT-4o, and \deepseek on \bestof{1}. The improvement (denoted as $\Delta$) is measured against the baseline (w/o refinement).}
    \resizebox{\linewidth}{!}{
      \begin{tabular}{cccccccc}
      \toprule
      \multirow{2}[6]{*}{\textbf{LLMs}} & \multirow{2}[6]{*}{\textbf{Methods}} & \multicolumn{6}{c}{\textbf{\bestof{1}}} \\
  \cmidrule(lr){3-8}        &       & \pctopt & $\Delta \uparrow$ & \speedup & $\Delta \uparrow$ & \pctcorrect & $\Delta \uparrow$ \\
      \midrule
      \midrule
       & Baseline (w/o refinement)  
            & 31.24\%  &     & 2.95$\times$  &    & 46.52\%  &\\
      \midrule
      
  \multirow{3}[1]{*}{\shortstack{\qwencoder 32B \\ \textsc{Instruct}}} 
  & Self Debugging & 35.69\%  & \textcolor{cadmiumgreen}{+4.45}  & 3.02$\times$  & \textcolor{cadmiumgreen}{+0.07}  & 53.74\%  & \textcolor{cadmiumgreen}{+7.22} \\
  
  & Direct Test Generation & 38.74\%  & \textcolor{cadmiumgreen}{+7.50}  & 3.08$\times$   & \textcolor{cadmiumgreen}{+0.13}  & 57.49\%  & \textcolor{cadmiumgreen}{+10.97} \\
  
  & \rowcolor{highlightcolor} \textbf{Anchor Verification}                          & 40.48\%  & \textcolor{cadmiumgreen}{+9.24}  & 3.17$\times$   & \textcolor{cadmiumgreen}{+0.22}  & 59.09\%  & \textcolor{cadmiumgreen}{+12.57} \\
            
  \midrule
      
  \multirow{3}[2]{*}{GPT-4o} 
          
      & Self Debugging & 37.47\%  & \textcolor{cadmiumgreen}{+6.23}  & 3.06$\times$  & \textcolor{cadmiumgreen}{+0.11}  & 55.65\%  & \textcolor{cadmiumgreen}{+9.13} \\
  
      & Direct Test Generation & 39.64\%  & \textcolor{cadmiumgreen}{+8.40}  & 3.13$\times$   & \textcolor{cadmiumgreen}{+0.18}  & 57.86\%  & \textcolor{cadmiumgreen}{+11.34} \\
  
      & \rowcolor{highlightcolor} \textbf{Anchor Verification}                          & 42.50\%  & \textcolor{cadmiumgreen}{+11.26}  & 3.32$\times$  & \textcolor{cadmiumgreen}{+0.37}  & 63.60\%  & \textcolor{cadmiumgreen}{+17.08} \\
  
  \midrule
      
  \multirow{3}[1]{*}{\deepseek} 
      & Self Debugging & 40.61\%  & \textcolor{cadmiumgreen}{+9.37}  & $3.23\times$  & \textcolor{cadmiumgreen}{+0.28}  & 59.62\%  & \textcolor{cadmiumgreen}{+13.10} \\
      
      & Direct Test Generation  & 40.17\%  &                          \textcolor{cadmiumgreen}{+8.93}  & 3.18$\times$  & \textcolor{cadmiumgreen}{+0.23}  & 58.73\%  & \textcolor{cadmiumgreen}{+12.21} \\
      
      & \rowcolor{highlightcolor} \textbf{Anchor Verification}                          & \textbf{47.28\%}  & \textcolor{cadmiumgreen}{\textbf{+16.04}}  & \textbf{3.40$\times$}  & \textcolor{cadmiumgreen}{\textbf{+0.45}}  & \textbf{65.32\%}  & \textcolor{cadmiumgreen}{\textbf{+18.80}} \\
  
      \midrule
      \midrule
       & Baseline (w/o refinement)  
            & 58.90\%  &     & 5.22$\times$  &    & 61.55\%  &\\
      \midrule
      
  \multirow{3}[1]{*}{\shortstack{\qwencoder 32B \\ \textsc{Instruct}}} 
  & Self Debugging & 58.42\%  & \textcolor{red}{-0.48}  & 5.13$\times$  & \textcolor{red}{-0.09}  & 61.14\%  & \textcolor{red}{-0.41} \\
  
  & Direct Test Generation & 62.98\%  & \textcolor{cadmiumgreen}{+4.08}  & 5.46$\times$   & \textcolor{cadmiumgreen}{+0.24}  & 65.95\%  & \textcolor{cadmiumgreen}{+4.40} \\
  
  & \rowcolor{highlightcolor} \textbf{Anchor Verification}                          & 64.75\%  & \textcolor{cadmiumgreen}{\textbf{+5.85}}  & 5.67$\times$   & \textcolor{cadmiumgreen}{\textbf{+0.45}}  & 67.28\%  & \textcolor{cadmiumgreen}{\textbf{+5.73}} \\
            
  \midrule
      
  \multirow{3}[2]{*}{GPT-4o} 
          
      & Self Debugging & 61.96\%  & \textcolor{cadmiumgreen}{+3.06}  & 5.59$\times$  & \textcolor{cadmiumgreen}{+0.37}  & 63.60\%  & \textcolor{cadmiumgreen}{+2.05} \\
  
      & Direct Test Generation & 65.43\%  & \textcolor{cadmiumgreen}{+6.53}  & 5.71$\times$   & \textcolor{cadmiumgreen}{+0.49}  & 68.61\%  & \textcolor{cadmiumgreen}{+7.06} \\
  
       & \rowcolor{highlightcolor} \textbf{Anchor Verification}                          & 68.40\%  & \textcolor{cadmiumgreen}{\textbf{+9.50}}  & 5.90$\times$  & \textcolor{cadmiumgreen}{\textbf{+0.68}}  & 71.98\%  & \textcolor{cadmiumgreen}{\textbf{+10.43}} \\
  
  \midrule
      
  \multirow{3}[1]{*}{\deepseek} 
      & Self Debugging & 64.11\%  & \textcolor{cadmiumgreen}{+5.21}  & $5.63\times$  & \textcolor{cadmiumgreen}{+0.41}  & 65.64\%  & \textcolor{cadmiumgreen}{+4.09} \\
      
      & Direct Test Generation  & 66.26\%  &                          \textcolor{cadmiumgreen}{+7.36}  & 5.81$\times$  & \textcolor{cadmiumgreen}{+0.59}  & 69.53\%  & \textcolor{cadmiumgreen}{+7.98} \\
      
      & \rowcolor{highlightcolor} \textbf{Anchor Verification (ours)}                          & \textbf{71.06\%}  & \textcolor{cadmiumgreen}{\textbf{+12.16}}  & \textbf{6.08$\times$}  & \textcolor{cadmiumgreen}{\textbf{+0.86}}  & \textbf{74.54\%}  & \textcolor{cadmiumgreen}{\textbf{+12.99}} \\
  
  \bottomrule
      \end{tabular}
      }
    \label{tab:anchor_pie}
  \end{table*}%

==> tables/root.tex <==
\begin{figure}[h]
    \centering
    \begin{minipage}{0.47\textwidth}
        \centering
        \tabcaption{xxx1}
        {\small
        \begin{tabular}{cccc}
            \toprule
            \multirow{2}{*}{LLMs} & \multicolumn{3}{c}{bestof{1}} \\
             \cmidrule(lr){2-4} & pctopt & speedup & pctcorrect \\
            \midrule
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
        \bottomrule
            \end{tabular}
        }
    \end{minipage}\hfill
    \begin{minipage}{0.51\textwidth}
        \tabcaption{xxx2}
        \centering
        {\scriptsize
        \begin{tabular}{cccc}
            \toprule
            \multirow{2}{*}{LLMs} & \multicolumn{3}{c}{bestof{1}} \\
             \cmidrule(lr){2-4} & pctopt & speedup & pctcorrect \\
            \midrule
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
            base & 58.90\% & 5.22 & 61.55\% \\
        \bottomrule
            \end{tabular}
        }
    \end{minipage}
\end{figure}
